Best of Both Worlds Policy Optimization

Policy optimization methods are popular reinforcement learning algorithms in practice. Recent works have built theoretical foundation for them by proving $\sqrt{T}$ regret bounds even when the losses are adversarial. Such bounds are tight in the worst case but often overly pessimistic. In this work, we show that in tabular Markov decision processes (MDPs), by properly designing the regularizer, the exploration bonus and the learning rates, one can achieve a more favorable polylog$(T)$ regret when the losses are stochastic, without sacrificing the worst-case guarantee in the adversarial regime. To our knowledge, this is also the first time a gap-dependent polylog$(T)$ regret bound is shown for policy optimization. Specifically, we achieve this by leveraging a Tsallis entropy or a Shannon entropy regularizer in the policy update. Then we show that under known transitions, we can further obtain a first-order regret bound in the adversarial regime by leveraging the log-barrier regularizer.

==> small-loss.tex <==
\section{Small Loss Bound (Known transition)}

\begin{algorithm*}[t]
\caption{Policy Optimization (Template)} \label{alg: template smallloss}
    \textbf{Define}: $\psi_t(\pi;s)$ and $b_t(s)$ are defined according to \pref{fig: psi and b choices}.   \\
    \textbf{Define}: $  \gamma_t=\frac{1700H^4A}{t}$.   \\
    \For{$t=1,2,\ldots$}{
        \begin{align}
            \pi_{t}(\cdot|s) = \argmin_{\pi\in\Delta_A}\left\{ \sum_{\tau=1}^{t-1} \sum_a \pi(a)\left(\hatQ_\tau(s,a) - B_\tau(s,a) - C_\tau(s,a)\right) +   \psi_t(\pi;s)\right\}   \label{eq: pi_t def}
        \end{align}
        \If{$\exists s,a$ such that $\frac{\eta_t(s,a)}{\mu_t(s)}>$}{
            Include a virtual episode with $L=0$ and let 
            \begin{align*}
                b_t(s) = \sum_{a}\left(\frac{1}{\eta_{t+1}(s,a)} - \frac{1}{\eta_t(s,a)}\right)\log T
            \end{align*}
            where 
            \begin{align*}
                \eta_{t+1}(s,a) = \max\left\{\frac{\mu_t(s)}{2\text{poly}(H)}, \ \ \frac{\eta_t(s,a)}{1+\frac{1}{A\log T}}\right\}
            \end{align*}
        }
        
        Execute $\pi_t$ in episode $t$, and receive $\{\ell_t(s_{t,h}, a_{t,h})\}_{h=0}^{H-1}$. \\
        \ \\
        \textbf{Define $\calP_t$: }
        For the unknown transition case, update the confidence set: 
        \begin{align}
            \calP_t &= \Bigg\{\tildeP:~~  \tildeP(\cdot|s,a)\in\Delta(\calS), ~~ \left|\tildeP(s'|s,a) - \hatP_t(s'|s,a)\right|\leq 2\sqrt{\frac{\hatP_t(s'|s,a)]\iota}{n_t(s,a)}} + \frac{14\iota}{3n_t(s,a)}, \nonumber \\
            &\qquad \qquad ~~ \forall (s,a,s')\in \calS_h\times \calA\times \calS_{h+1},~~\forall h\in\{0,1,\ldots, H-1\}\Bigg\}. \label{eq: definition of transition P}
        \end{align}
        For the known transition case, define $\calP_t=\{P\}$. \\
        \ \\
        \textbf{Define $\hatQ_t$: }
        For $s\in\calS_h$, let $\ind_t(s,a)=\ind\{(s_{t,h},a_{t,h})=(s,a)\}$,  
        $L_{t,h} = \sum_{h'=h}^{H-1} \ell_t(s_{t,h'}, a_{t,h'})$, and 
        \begin{align}
            \hatQ_t(s,a) = \frac{\ind_t(s,a)L_{t,h}}{\mu_t(s)\pi_t(a|s)}, \qquad \text{where\ }  \mu_t(s) =  \overline{\mu}_t^{\pi_t}(s) + \gamma_t.  \label{eq: hatQ def} 
        \end{align}
        \textbf{Define $C_t$: }
Let $c_t(s)=\frac{\mu_t(s) - \underline{\mu}_t^{\pi_t}(s)}{\mu_t(s)}H$, and  $C_t(s,a)$ satisfy
         \begin{align}               
           C_t(s,a)&=\max_{\tildeP\in\calP_t}\E_{s'\sim \tildeP(\cdot|s,a), a'\sim \pi_t(\cdot|s')}\Big[c_t(s') + C_t(s',a')\Big], \label{eq: C def}  % \nonumber \\
           % C_t(s,a) &= c_t(s,a) + \max_{\tildeP\in\calP_t}\E_{s'\sim \tildeP(\cdot|s,a), a'\sim \pi_t(\cdot|s')}\left[C_t(s',a')\right].   
        \end{align} 
        
        \textbf{Define $B_t$: } Let $B_t(s,a)$ satisfy
        \begin{align}
             & B_t(s,a) =  \max_{\tildeP\in \calP_t}\E_{s'\sim \tildeP(\cdot|s,a), a'\sim \pi_t(\cdot|s')}\left[b_t(s') +  \left(1+\frac{1}{H}\right) B_t(s',a')\right].  \label{eq: dil bonus alg} 
        \end{align}
    }
\end{algorithm*}
\begin{framed}
\textbf{Log barrier}: 
   \begin{align*}
            \psi_{t}(\pi;s) &= \sum_a \frac{1}{\eta_t(s,a)}\ln \frac{1}{\pi(a)}, \\
            b_t(s) &=  \sum_a\left[\left(\frac{1}{\eta_t(s,a)} - \frac{1}{\eta_{t-1}(s,a)}\right)\log(T) +  \frac{\eta_t(s,a)\phi_t(s,a)}{\mu_t(s)^2} \right] + \nu_t(s),
    \end{align*}
    where
        \begin{align*}
            \eta_{t}(s,a) &= \frac{1}{H^2A + \sqrt{\sum_{\tau=1}^{t-1} \frac{\phi_\tau(s,a)}{\mu_\tau(s)^2}}  }, \\
            \phi_t(s,a) &= \big(\ind_t(s,a)L_t(s,a) - \pi_t(a|s)\ind_t(s)L_t(s)\big)^2, \\
            \nu_t(s) &= \sum_a \eta_t(s,a)\pi_t(a|s)C_t(s,a)^2. 
        \end{align*}
\end{framed}

\begin{lemma}
    In all rounds, $\eta_t(s,a)\pi_t(a|s)B_t(s,a)\leq \frac{1}{H}$. 
\end{lemma}

\begin{proof}
    In real rounds, 
    \begin{align*}
        b_t(s) = \sum_a \frac{\eta_t(s,a)\ind_t(s,a)L_t(s,a)^2}{\mu_t(s)^2} \leq H^2\times \max_a \frac{\eta_t(s,a)}{\mu_t(s)}\times \frac{1}{\mu_t(s)} \leq \frac{1}{HS\mu_t(s)}. 
    \end{align*}
    Therefore, 
    \begin{align*}
        B_t(s,a) &= \sum_{s'} \mu^{\pi_t}(s'|s,a)b_t(s') \leq \sum_{s'} \mu^{\pi_t}(s'|s,a)\times \frac{1}{HS(\mu^{\pi_t}(s)\pi_t(a|s) \mu^{\pi_t}(s'|s,a) + \gamma_t)} \\
        &\leq \sum_{s'}  \frac{1}{HS(\mu^{\pi_t}(s)\pi_t(a|s) + \gamma_t)} \\
        &\leq \frac{1}{H\mu_t(s)\pi_t(a|s)}
    \end{align*}
    and thus
    \begin{align*}
        \eta_t(s,a)\pi_t(a|s)B_t(s,a)\leq \frac{1}{H}\frac{\eta_t(s,a)}{\mu_t(s)} \leq \frac{1}{H}. 
    \end{align*}
    
    In virtual rounds, 
    \begin{align*}
        b_t(s) \leq  \sum_a \left(\frac{1}{\eta_{t+1}(s,a)} - \frac{1}{\eta_t(s,a)}\right)\log(T)\leq \sum_{a}\frac{\log T}{A\log T} \leq 1
    \end{align*}
    so 
    \begin{align*}
        \eta_t(s,a)\pi_t(a|s)B_t(s,a)\leq \eta_t(s,a)H\leq \frac{1}{H}. 
    \end{align*}
\end{proof}

\begin{lemma}
    $\frac{\pi_{t+1}(a|s)}{\pi_t(a|s)}\in [1-\frac{1}{2H}, 1+\frac{1}{2H}]$ and thus $\frac{\mu_{t+1}(s)}{\mu_t(s)}\in[\frac{1}{2},\frac{3}{2}]$. 
\end{lemma}
\begin{proof}
   By the analysis of log-barrier FTRL, 
   \begin{align*}
       \sum_a \frac{(\pi_{t+1}(a|s) - \pi_t(a|s))^2}{\pi_t(a|s)^2 \eta_t(s,a)} \leq \sum_a \eta_t(s,a) \pi_t(a|s)^2 B_t(s,a)^2 \leq \frac{1}{4H^2}. 
   \end{align*}
   \cw{the last inequality doesn't hold unless we use $\eta_t(s)$ but not $\eta_t(s,a)$. How to use coordinate-dependent learning rate? (or do we really need this lemma? )}
\end{proof}

%\begin{lemma}
%   The number of virtual episodes is upper bounded by 
%\end{lemma}
%\begin{proof}
%   Each time the virtual round happen, there exists $s,a$ such that 
%   either 
%   \begin{align*}
%       \frac{\eta_{t+1}(s,a)}{\mu_{t+1}(s)} \leq \frac{2\eta_{t+1}(s,a)}{\mu_t(s)}= \frac{1}{poly(H)}. 
%   \end{align*}
%   or 
%   \begin{align*}
%       \frac{1}{\eta_{t+1}(s,a)} - \frac{1}{\eta_t(s,a)} = \frac{1}{A\log T}. 
%   \end{align*}
%   If all $s,a$ satisfies the first, then the next round will not be 
%\end{proof}

\begin{lemma}

\end{lemma}
\begin{proof}
    \begin{align*}
        \sum_{t=1}^T V^{\pi_t}(s_0; b_t)
        &\leq \sum_{t=1}^T\sum_s \mu^{\pi_t}(s)b_t(s)  \\
        &\leq \sum_{t: \text{real}}\sum_s \mu^{\pi_t}(s)\frac{\frac{\phi_t(s,a)}{\mu_t(s)^2} + \frac{\phi_{t-1}(s,a)}{\mu_{t-1}(s)^2}}{ \sqrt{\sum_{\tau=1}^{t-1} \frac{\phi_\tau(s,a)}{\mu_\tau(s)^2}}  } + \sum_{t:\text{virtual}}\sum_s \mu^{\pi_t}(s)\times 1
    \end{align*}
\end{proof}

==> tabular.tex <==








==> tabular2.tex <==
\section{123}
